An Independent Measure of the Kinematic Dipole from SDSS

We utilize the Sloan Digital Sky Survey (SDSS) extended Baryon Oscillation Spectroscopic Survey (eBOSS) and Baryon Oscillation Spectroscopic Survey (BOSS) catalogs with precise spectroscopic redshifts to estimate the kinematic redshift dipole caused by the proper motion of the Solar system. We find that the velocity extracted from the kinematic dipole is consistent with Cosmic Microwave Background inferred values. Although the small sky coverage and limited number density of the SDSS sources constrain us from obtaining precise and robust measurements, we leverage the redshift dipole method to estimate the kinematic dipole. The velocity measurements in this study are insensitive to intrinsic clustering, associated with the source count dipole. The kinematic dipole measured in this work and its consistency with CMB values do not guarantee isotropy at large scales. The anisotropy (excess dipole) measured with the NRAO VLA Sky Survey (NVSS) and the WISE Catalog (CatWISE) could be due to the intrinsic distribution of galaxies. The results in this work focus solely on the kinematic dipole term.

==> def.tex <==
\usepackage[ngerman,english]{babel}
\newif\ifAMStwofonts
\AMStwofontstrue 
\def\degr{\hbox{$^\circ$}}
\def\arcmin{\hbox{$^\prime$}}
\def\arcsec{\hbox{$^{\prime\prime}$}}
\def\vgrad{{\bf \nabla}}
\def\pesc{{\rm P}_{\rm esc}}
\def\fsnr{{\rm f}_{\rm _{SNR}}}
\def\aobs{{\alpha_{\rm _{obs}}}}
\def\baobs{{{\bar\alpha}_{\rm _{obs}}}}
\def\bz{{b(z)}}
\def\nz{{N(z)}}
\def\cl{{C_\ell}}
\def\cln{{C^n_\ell}}
\def\clth{{C^{\rm th}_\ell}}
\def\clobs{{C^{\rm obs}_\ell}}
\def\clcorr{{C^{\rm corrected}_\ell}}
\def\dl{{d_{\ell m}}}
\def\al{{a_{\ell m}}}
\def\almo{{a^{\rm obs}_{\ell m}}}
\def\tal{{{\tilde a}_{\ell m}}}
\def\dl{{d_{\ell m}}}
\def\vPsi{{\bf \Psi}}
\def\vPhi{{\bf \Phi}}
\def\vmu{{\bm \mu}}
\def\wpdot{W_{{\dot \phi}}}
\def\wph{W_{ \phi}}
\def\wv{W_{ \rm V}}
\def\cA{${\cal A}$}
\def\caM{{\cal M}}
\def\rmin{{r_{_{\rm min}}}} 
\def\rmax{{r_{_{\rm max}}}} 
\def\rz{{r}} 
\def\vh{{v_{_{\rm h}}}} 
\def\Vs{{V_{_{\rm seed}}}} 
\def\Vsi{{V_{_{{\rm seed},i }   }}} 
\def\As{{a_{_{\rm seed}}}} 
\def\Asj{{a^j_{_{\rm seed}}}} 
\def\zcos{z_{_{\rm cos}}}
\def\Ps{{P_{_{\rm seed}}}} 
\def\Psii{{P_{_{{\rm seed},i} }}} 
\def\sigint{\sigma_{\eta,{\rm int}}}
%\def\ssigint{\sigma^2_{\eta,{\rm int}}}
\def\ssigint{\sigma^2_{\eta}}
\def\cBo{{\cal B}_{\rm o}}
\def\cBt{{\cal B}_{\rm t}}
\def\Pm{{P_{_{\rm m}}}} 
\def\ti{{t_{_{0}}}} 
\def\Pa{{P_{_{\alpha}}}} 
\def\Qks {{Q_{_{\rm KS}}}} 
\def\rcu{ {r_{_{\rm cut}} }}
\def\md{ {M_{_{\rm disk}} }}
\def\psid{ {\Psi_{_{\rm disk}} }}
\def\psih{ {\Psi_{_{\rm halo}} }}
\def\kpc{ {\; {\rm kpc}}}
\def\Ns{N_{\rm s}}
\def\caH{{\cal H}}
\def\fg{{f_{_{\rm g} }}}
\def\fdm{{f_{_{\rm DM} }}}
\def\fgz{{f_{_{\rm g17} }}}
\def\etaz{{\eta_{_{\rm 01} }}}
\def\caS{{\cal S}}
\def\wp{{w_{+}}}
\def\wm{{w_-}}
\def\mup{{\mu_+}}
\def\sigmatwo{{\sigma_{_{2}}}}
\def\mum{{\mu_-}}
\def\nup{{\nu_+}}
\def\num{{\nu_-}}
\def\lp{{\lambda_+}}
\def\lm{{\lambda_-}}
\def\vnabla{\bm{\nabla}}
\def\vv{\bf v}
\def\vu{\bf u}
\def\vB{{\bf B}}
\def\eeth{ E_{_{\rm th}} } 
\def\mm{M_{\rm m}}
\def\ms{M_{\rm s}}
\def\Vp{{V_+}}
\def\Vm{{V_-}}
\def\gsim{~\rlap{$>$}{\lower 1.0ex\hbox{$\sim$}}}
\def\xm{x_{_{\rm M}}}
\def\tdmj{{\tilde \varrho}_{{\rm M}j}}
\def\td{t_{_{\rm d}}}
\def\tobs{t_{_{\rm obs}}}
\def\simpropto{\lower.2ex\hbox{$\; \buildrel \propto \over \sim \;$}}
\def\ltsim{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\gtsim{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\ltsim{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\gtsim{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\th{\theta}
\def\tht{\tilde \theta}
\def\cv{ v}
\def\cvt{ \tilde v}
\def\wt{ \tilde w}
\def\ut{ \tilde u}
\def\dotr{\dot {\bf r}}
\def\ni{\noindent}
\def\gm{\gamma}
\def\pa{\partial}
\def\vm{{\langle v_{12}\rangle_{{\rm m}} }} 
\def\vg{v_{_{\rm g}}}
\def\ag{a_{_{\rm g}}}
\def\aitf{a_{_{\rm itf}}}
\def\vmle{\vB_{_{\rm MLE}} }
\def\vace{\vB_{_{\rm ASCE}} }
\def\vF{{\bf F}}
\def\Rv{R_{\rm v}}
\def\vnabla{{\bf \nabla}}
\def\gmp{\gamma_\|}
\def\gmt{\gamma_\perp}
\def\sgt{\sigma_\perp}
\def\sgls{\sigma_{ls}}
\def\bfeta{{\bf \eta}}
\def\stream{{\langle v_{12}(r)\rangle}}   
\def\H{{\cal H}}
\def\He{{\cal H}{\rm e}}
\def\za{{Zel'dovich approximation}}
\def\cm{\,{\rm cm}}
\def\erg{\,{\rm erg}}
\def\Hz{\,{\rm Hz}}
\def\sr{\,{\rm sr}}
\def\s{\,{\rm s}}
\def\K{\,{\rm K}}
\def\sv{\Theta{^{\rm V}}}
\def\sw{\Theta{^{\rm \Phi}}}
\def\sisw{\Theta{^{\rm { \dot \Phi}}}}
\def\tsv{{\tilde \Theta}{^{\rm V}}}
\def\tsw{{\tilde \Theta}{^{\rm \Phi}}}
\def\tsisw{{\tilde \Theta}{^{\rm { \dot \Phi}}}}
\def\sun{\Theta_{_{\rm un}}}
\def\fsk{f_{_{\rm sky}}}
  \def\rg{\rho_{_{\rm g}}}
    \def\rdm{\rho_{_{\rm dm}}}
\def\kms{\mbox{km\,s$^{-1}$}}
\newcommand{\Mpc}{\, {\rm Mpc} }
\def\Msol{\mbox{M$_\odot$}}
%\def\mg{\mbox{M$_{\rm g}$}}
%\def\mbh{\mbox{M$_{\rm bh}$}}
%\def\mp{\mbox{M$_{\rm p}$}}
%\def\mg{ M_{_{\rm g}} }
%\def\mbh{ M_{_{\rm BH}} }
%\def\mbht{ M_{_{\rm BH,8 }} }
\def\mg{ M_{{ g}} }
\def\mbh{ M_{{BH}} }
\def\mbht{ M_{{ BH,8 }} }
%\def\mdm{ M_{_{\rm DM}} }
\def\mdm{ M_{{DM}} }
\def\prd{Physical Review D.}
\def\nat{Nature}
\def\astjo{Astronomical Journal}
\def\mp{ m_{_{\rm p}} }
\def\sigT{ \sigma_{_{\rm T}} }
\def\bigexpec#1{\biggl \langle#1\biggl \rangle}
\def\expec#1{\langle#1\rangle}
\def\dd{\,{\rm d}}
\def\dhik{(n_{{_{\rm HI}}})_{k}}
\def\rb{{R_{_{\rm b}}}}
\def\gammab{\gamma_{_{\rm b}}}
\def\vb{{v_{_{\rm b}}}}
\def\nb{{n_{_{\rm b}}}}
\def\rs{{r_{_{\rm s}}}}
\def\ngal{{n_{_{\rm gal}}}}
\def\bnb{{{\bar n}_{_{\rm b}}}}
\def\pb{{p_{_{\rm b}}}}
\def\pam{{p_{_{\rm a}}}}
\def\eb{{E_{_{\rm b}}}}
\def\ebi{{E_{_{\rm bi}}}}
\def\pbi{{p_{_{\rm bi}}}}
\def\rbi{{R_{_{\rm bi}}}}
\def\rhob{{\rho_{_{\rm b}}}}
\def\rhov{{\rho_{_{\rm v}}}}
\def\gN{g_{_{\rm N}}}
\def\gM{g_{_{\rm M}}}
%\parskip 6pt
%\overfullrule = 0pt
\def\np{\vfill\eject}
\def\no{\noindent}
\def\bk{\hfill\break}
%       The following macros should be used only in math mode.
\def\ergcms{\,{\rm erg\,cm^{-3}\,s^{-1}}}
\def\kms{\ {\rm km\,s^{-1}}}
\def\hmpc{\ {\rm h^{-1}Mpc}}
\def\hh{\ {\rm h_{50}}}
\def\hmmpc{\ {\rm h\,Mpc^{-1}}}
\def\gcc{\,{\rm g\,cm^{-3}}}
\def\tl{ {\tilde l}}
\def\pcc{\,{\rm cm^{-3}}}
\def\kel{\,{\rm K}}
\def\dd{{\rm d}}
\def\nb{{\bar n}}
\def\ln{{\rm ln}}
\def\pa{\partial}
\def\rarrow{\rightarrow}
\def\larrow{\leftarrow}
%\def\la{\langle}
%\def\ra{\rangle}
\def\grad{\nabla}
%
\def\pmb#1{\setbox0=\hbox{#1}%
\kern-.025em\copy0\kern-\wd0
\kern.05em\copy0\kern-\wd0
\kern-.025em\raise.0433em\box0}
\def\th{\vartheta}
%\def\vth{\vec\th}
\def\vth{\pmb{$\th$}}
\def\ph{\varphi}
 \def\disw{\Theta_{_{\rm  ISW}}}

\def\phv{\ph_v}
\def\phg{\ph_g}
\def\vV{\pmb{V}}
\def\vv{\pmb{v}}
\def\vL{\pmb{L}}

\def\vs{\pmb{s}}
\def\vq{\pmb{q}}
\def\vx{\pmb{x}}
\def\vr{\pmb{r}}
\def\vn{\pmb{n}}
\def\hvn{\hat {\vr}}

%\def\vg{\pmb{$g$}}
\def\vk{\pmb{k}}
\def\hvk{\hat {\vk}}
\def\vaj{\pmb{\alpha}}
\def\vpsi{\pmb{\psi}}
\def\phiv{\phi_v}
\def\phig{\phi_g}
\def\pot {\Phi}
\def\iras {{\it IRAS~}}
\def\velmod{VELMOD~}
%\def\Ft {{\         }}
%\def\tj {{\wpdot}}
\def\Ft {{F}}
\def\tj{{F}}

\def\ajj {{a}^j}
\def\aj{AJ}
\def\gh{\gamma_{_{*}}}  \def\ah{\alpha_{_{*}}}  \def\bh{\beta_{_{*}}}
\def\Nh{N_{_{*}}} 
\def\ajp {{\psi}^{j'}}
\def\ip {i^\prime}
\def\jp {j^\prime}
\def\bfr {{\bf r}}
\def\etal{{\it et al.\ }}
\def\con {5\log {\rm e}}
\def\simlt{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
\def\simgt{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\Msun{\rm\> M_{\odot}}
%\def\vnabla{\vec\nabla}
\def\vnabla{\pmb{$\nabla$}}
\def\vitf{v_{_{\rm itf} }}
\def\void#1{{#1}}
%\include{rotating}
\newcommand{\beq}{\begin{equation}}

\newcommand{\eeq}{\end{equation}}
\def\beqa{\begin{eqnarray}}
\def\eeqa{\end{eqnarray}}
%\def\la{\lower.5ex\hbox{$\; \buildrel < \over \sim \;$}}
%\def\ga{\lower.5ex\hbox{$\; \buildrel > \over \sim \;$}}
\def\fixit#1{}
\def\hmpc{h^{-1}\,{\rm Mpc}}
\def\hkpc{h^{-1}\,{\rm kpc}}
\def\dd{{\rm d}}
\def\apj{ApJ}
\def\jcap{JCAP}
\def\prl{Physical Review Letters}
\def\astroj{Astrophysical. J}
\def\aapr{A\&A Rev.}
\def\aaps{A\&AS}
\def\apjs{ApJ. S}
\def\cN{{\cal N}}
\def\cn{{\cal n}}
\def\cS{{\cal S}}
\def\physrep{Physics Reports}
\def\apjl{ApJL}
\def\mnras{MNRAS}
\def\aap{A\&A}
\def\araa{ARAA}
\def\prd{Physical Review D.}
\def\nat{Nature}
\def\apjl{ApJL}
\def \ssr{Space Science Reviews}

%\usepackage{lscape}
%\input{definitions}

\def\file#1{\texttt{#1}}
\def\mudm{\mu_{_{\delta\! M_*}}}
\def\sigdm{\sigma_{_{\delta\! M_*}}}
\def\mual{\mu_{_{\delta\! \alpha}}}
\def\sigal{\sigma_{_{\delta\! \alpha}}}

\def\muas{  \mu  as}
\def\muasyr{\mu as \, {\rm yr}^{-1} }


